DiPair: Fast and Accurate Distillation for Trillion-Scale Text Matching and Pair Modeling

Pre-trained models like BERT (Devlin et al., 2018) have dominated NLP / IR applications such as single sentence classification, text pair classification, and question answering. However, deploying these models in real systems is highly non-trivial due to their exorbitant computational costs. A common remedy to this is knowledge distillation (Hinton et al., 2015), leading to faster inference. However -- as we show here -- existing works are not optimized for dealing with pairs (or tuples) of texts. Consequently, they are either not scalable or demonstrate subpar performance. In this work, we propose DiPair -- a novel framework for distilling fast and accurate models on text pair tasks. Coupled with an end-to-end training strategy, DiPair is both highly scalable and offers improved quality-speed tradeoffs. Empirical studies conducted on both academic and real-world e-commerce benchmarks demonstrate the efficacy of the proposed approach with speedups of over 350x and minimal quality drop relative to the cross-attention teacher BERT model.

==> intro2.tex <==

% \section{Introduction (KR)}

% % Present the introduction in a logical way and clear way

% %1. What is the task and Why it is important
% % Present the importance of semantic matching with pairwise textual input for many IR/NLP tasks.
% Modeling the relationship between textual objects is critical to numerous NLP and information retrieval (IR) applications \cite{10.5555/2683840}. This subsumes a number of different problems such as textual entailment, semantic text matching, paraphrase identification, plagiarism detection and relevance modeling. For example, modeling the relationship between queries and documents / keywords is central to search engine / digital advertisement systems \cite{10.5555/2683840,DBLP:journals/corr/abs-1903-06902}.

% %2. What is the current approach and problems/missing parts of current state-of-art work
% % 2.1 Review  the existing works on neural semantic matching models: representation-focused models (Dual Encoder models), interaction-focused models and the recent Transformer/BERT based methods
% Recently neural network based models have demonstrated large gains in this space \cite{DBLP:conf/nips/HuLLC14,DBLP:conf/aaai/PangLGXWC16}. In particular the Transformer/ BERT family of models \cite{devlin2018:bert,albert19,roberta19,electra20}) have set the new bar for these semantic matching problems. However, the computational costs of these models have proven to be prohibitively expensive, thus limiting their use in real-world applications \cite{FC19}. For example on an ecommerce relevance-scoring task (the \ptdata~data -- Sec. \ref{sec:result-on-p2t-data}), scoring the (trillion+) relevance would take years.

% % 2.2 Why knowledge distillation is important for serving BERT based models
% One popular remedy is to distill these expensive \emph{teacher} models \cite{DBLP:journals/corr/HintonVD15} into lightweight \emph{student} models. Training these \emph{students} using examples labeled by the \emph{teacher} has been shown to maintain quality while enabling faster inference. Key to the effectiveness of distillation techniques is a good trade-off between student quality and inference speed. 

% However, as we show here, existing knowledge distillation techniques \cite{DBLP:journals/corr/abs-1910-01108,DBLP:journals/corr/abs-1909-10351,DBLP:journals/corr/abs-1908-08962,DBLP:journals/corr/abs-1903-12136} fall short on the quality-speed trade-off when dealing with pairs of texts. On one hand, approaches that model the texts jointly (\emph{i.e.}, using cross-attention) even one as highly optimized as \berttiny~\cite{DBLP:journals/corr/abs-1908-08962} are still order of magnitude(s) too slow. 

% % 2.3.2 Cosine/dot based dual encoder models are very efficient. But the matching performance is bad.
% On the other hand, lie techniques that model the texts independently such as the ``Dual Encoder''  models\footnote{These \emph{two-tower} encode the two texts separately and then combine them via a lightweight dot product / cosine.} \cite{JDH17,SL14,DII+04,HYH+18,GKC+,WGS+}.
% By exploiting the independence of the texts, these techniques can significantly speed up inference by caching/indexing the embeddings of individual texts.
% However this speedup comes at a significant cost -- with sharply reduced performance.

% % Consider dropping this example / para if we don't have space / move elsewhere
% The key drawback here is that these independent models lack the ability to mimic the cross-attention enabled teachers and model the joint nuances and facets of the texts.
% As a motivating example, consider the ecommerce term relevance-scoring task. For the product ``Black Sport Nike Shoes for Boys Size Wide", terms such as ``black", ``wide footwear" and ``nike shoes" are all relevant. However enforcing similarity between the independently modeled term and product, will lead to the embeddings of ``black" and ``nike shoes" being incorrectly considered as similar to each other.



% % 3. What is our contribution/findings/ the novel parts of the model or architecture/   

% Motivated by this, we propose \textbf{DiPair} for fast and accurate distillation of large-scale text pairs. DiPair aims to combine the best of both worlds: Like dual-encoder models it leverages common pre-computation while at the same time models the text jointly -- with cross-attention -- using multiple contextual embedding for each text. In particular we concatenate a small fraction of the output token embeddings from each text, and then jointly model this smaller ``sequence'' using a transformer \emph{head}.
% We demonstrate that a two-stage, end-to-end training allows the proposed DiPair model to learn a richer multifaceted semantic representations of the text pairs. The resulting DiPair model is 350x+ faster with minimal quality drop relative to the teacher on both academic and real-world datasets. 

% % 4 Summarize the contribution of this work
% % DiPair technique: Fast and good quality
% % two stage training with more quality control knobs
% % Need for attention based students
% In summary, our main contributions include:
% \begin{itemize}
% \itemsep0em
%     \item \textbf{DiPair}: A new framework for distilling fast, accurate models on text pair tasks. Its advantages include: 1) Generic framework applicable across numerous applications involving pairwise/n-ary textual input. To the best of our knowledge this is the first work tackling this problem. 2) Highly practical solution with limited storage and computation needs that scales to trillions of examples. 3) Large speedups for model inference -- 350x+ faster relative to teacher and 8x faster than previous best \cite{DBLP:journals/corr/abs-1908-08962}.
%     \item Novel two-stage, end-to-end training scheme enables an  improved quality-speed tradeoff curve as shown in Fig.~\ref{fig:dipair-tradeoff}.
%     \item Evidence that (self and cross) attention is important for student models when it comes to distilling from teachers like BERT.
%     \item Extensive experimentation on academic and real-world (ecommerce) datasets demonstrate that DiPair can lead to fast, effective models that outperform existing techniques.
% \end{itemize}

% \begin{figure}[t]
%     \centering
%     \vspace{-0.1em}
%     \includegraphics[width=1.1\columnwidth]{fig/dipair-tradeoff.jpg}
%     \vspace{-1em}
%     \caption{Inference speed vs Quality tradeoff for the proposed DiPair technique relative to existing techniques on the \qpdata~dataset.}
%     \label{fig:dipair-tradeoff}
%     \vspace{-.5em}
% \end{figure}

\section{Methodology}

% Problem setting:

% Mention we focus on learning from weak labels — can be used for retraining but we focus on distillation

% Two tower models

% - Text pairs, full cross-attention and dual encoders
%     - Introduce some notation
%     - How dual encoders work
% - Our proposal: DiPair
%     - High-level overview
%     - Key aspects:
%         - The head
%         - Speeding up approach:
%             - Projection layer
%             - Truncated sequences
%     - Algorithm and two-staged training
%     - Comment: Generality
%         - Multiple losses
%         - Further extensions
%         - Any text pair task

